Efficient Straggler Replication in Large-scale Parallel Computing

In a cloud computing job with many parallel tasks, the tasks on the slowest machines (straggling tasks) become the bottleneck in the job completion. Computing frameworks such as MapReduce and Spark tackle this by replicating the straggling tasks and waiting for any one copy to finish. Despite being adopted in practice, there is little analysis of how replication affects the latency and the cost of additional computing resources. In this paper we provide a framework to analyze this latency-cost trade-off and find the best replication strategy by answering design questions such as: 1) when to replicate straggling tasks, 2) how many replicas to launch, and 3) whether to kill the original copy or not. Our analysis reveals that for certain execution time distributions, a small amount of task replication can drastically reduce both latency as well as the cost of computing resources. We also propose an algorithm to estimate the latency and cost based on the empirical distribution of task execution time. Evaluations using samples in the Google Cluster Trace suggest further latency and cost reduction compared to the existing replication strategy used in MapReduce.

==> tikz_macros.tex <==
\newcommand{\DWFIGWIDTH}{4cm}
\newcommand{\PGFDIR}{pgfplots}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{tikz}
\usetikzlibrary{arrows,shapes,decorations,shapes.misc,patterns}
\usetikzlibrary{calc,positioning,spy}
\usepackage{pgf}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\pgfplotsset{every axis/.append style={
            axis x line=bottom,
            axis y line=left,
            width = \DWFIGWIDTH,
            %height = 0.4\textwidth,
            %minor tick num=1,
            tick style={semithick},
            ticks=both,
            xmajorgrids,
            ymajorgrids,
            tick label style={font=\small},
            label style={font=\small},
            legend style={font=\small},
            title style={font=\small},
            }}
\usepgfplotslibrary{external}
\tikzexternalize%activate externalization
\tikzsetexternalprefix{tpdfs/}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{>=latex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfplotsset{dashdot/.style={dash pattern=on 1pt off 2pt on 6pt off 2pt}}
\pgfplotsset{tradeoffplot/.style={%
    xmin=3, 
    xmax=9.2,
    ymin=0, 
    ymax=73,
    xlabel={Cost},
    xlabel style={at={(1.1,0.05)}},
    ylabel={Latency},
    ylabel style={at={(0.1,1.05)}, rotate=-90},
    legend columns=1,
    legend style={ 
    at={(0.7,0.6)}, 
    cells={anchor=west},
    anchor=south 
    },
}}

% add pgfplot
\newcommand{\pgfplotwidth}[1]{\pgfplotsset{%
every axis/.append style={%
width={#1}}}}
\newcommand{\pgfplotheight}[1]{\pgfplotsset{%
every axis/.append style={%
height={#1}}}}
\newcommandx{\addpgfplot}[3][1=\DWFIGWIDTH,2=\PGFDIR]{%
\pgfplotwidth{#1}%
\tikzsetnextfilename{#3}%
\input{#2/#3}%
}
\newcommandx{\addpgfplotx}[3][1=\DWFIGWIDTH,2=\PGFDIR]{%
\pgfplotwidth{#1}%
\tikzset{external/force remake}%
\tikzsetnextfilename{#3}%
\input{#2/#3}%
}


